Pyramids and Extended Metric Measure Spaces

A pyramid is a generalisation of metric measure spaces (mm-spaces) introduced by M.~Gromov (Birkh\"auser 1999) to establish a geometric framework for measure-concentration problems. An extended metric measure space (emm-space) is another generalisation of mm-spaces introduced by Ambrosio--Gigli--Savar\'e (Invent.~Math.~2014) to extend Sobolev calculus and optimal transport theory to a broader extent. We prove that every pyramid has a representation by an emm-space through $1$-Lipschitz order. Furthermore, if pyramids are concentrated, this correspondence is unique up to isomorphism. This shows, for the first time, that all pyramids can be realised by concrete geometric spaces. Based on this representation, we introduce a new notion, a concentrated emm-space. We then define the observable distance for concentrated emm-spaces and establish three equivalent characterisations of concentration in terms of pyramids, Lipschitz observables and the observable distance. Furthermore, by developing an fibration approach, we show the $\Gamma$-$\limsup$ inequality of Cheeger energies as well as the stability of the log-Sobolev inequality and the Poincar\'e inequality under the weak convergence of pyramids associated with emm-spaces. Our results provide a new geometric approach for studying both the convergence of emm-spaces and concentration-of-measure phenomena across a broad class of infinite-dimensional models that have so far remained largely beyond the reach of existing geometric methods. Many of the significant examples arise in probability theory, including the Wiener space, the configuration space, Gaussian fields such as massive Gaussian free fields, spatial white noise and massive bi-Laplacian fields.

==> macro.tex <==
\RequirePackage{etex}
%% PACKAGES
\usepackage[english]{babel}
\usepackage[utf8]{inputenc}
\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{amssymb}
\usepackage{amsthm}
\usepackage{mathtools}
\usepackage{minitoc}
\usepackage{bbm}
\usepackage{braket}
\usepackage{enumerate}
\usepackage[inline]{enumitem}
\usepackage{esint}
\usepackage{varwidth}
\usepackage{tikz}
\usepackage{mathrsfs}
%\usepackage{thmtools}
\usepackage[hypertexnames=false]{hyperref}
\usepackage{enumitem}
\usepackage{cleveref}
\usepackage{autonum}
\usepackage{graphicx}
\usepackage[dvipsnames]{xcolor}

\newcommand{\LS}{\mathsf{LS}}
% \newcommand{\P}{\mathsf{P}}

\makeatletter
\newcommand{\tagsleft}{\tagsleft@true}
\newcommand{\tagsright}{\tagsleft@false}
\makeatother

% %%
% %% Pacchetti
% %%
% \usepackage[utf8]{inputenc}
% \usepackage[english] {babel}
% \usepackage{easyReview}
% \usepackage{mathrsfs}

% \usepackage[color]{showkeys}

% \usepackage{amsmath}
% \usepackage{amsfonts}
% \usepackage{amssymb}
% \usepackage{amsthm}
% \usepackage{mathtools}
% \usepackage{bbm,a4wide}

% \usepackage{braket}
% \usepackage{enumerate}
% \usepackage{esint}

% \usepackage[dvipsnames]{xcolor}%May be necessary if you want to color links
% % \usepackage[
% % 						%hidelinks,					%nasconde i link: antagonista di colorlinks (s 1 E no 2)
% % 						colorlinks,				%link a colori invece che riquadrati
% % 						breaklinks,unicode,
% % 						hypertexnames=false,
% % 						citecolor=OliveGreen,
% % 						linkcolor=Maroon
% % 						]{hyperref} 
                        
% \usepackage{hyperref}
% \hypersetup{
%     colorlinks=true, %set true if you want colored links
%     linktoc=all,     %set to all if you want both sections and subsections linked
%     linkcolor=Maroon,  %choose some color if you want links to stand out
%     citecolor=OliveGreen
% }


% %%
% %% TEOREMI ECC
% %%

% \theoremstyle{definition} \newtheorem{deff}{Definition} [section]
% \theoremstyle{definition} \newtheorem{prop} [deff]{Proposition}
% \theoremstyle{definition} \newtheorem{thm} [deff]{Theorem}
% \theoremstyle{definition} \newtheorem{lm} [deff]{Lemma}
% \theoremstyle{definition} \newtheorem{ass} [deff]{Assumption}


% \theoremstyle{remark} \newtheorem{es} [deff]{Example}
% \theoremstyle{remark} \newtheorem{rmk}[deff]{Remark} 
% \theoremstyle{plain} \newtheorem{cor}[deff]{Corollary} 

% \newtheoremstyle{claim}% Nome dello stile
%   {}% Spazio sopra
%   {}% Spazio sotto
%   {\itshape}% Font del corpo dell'enunciato
%   {}% Rientro del corpo dell'enunciato
%   {}% Font del titolo dell'enunciato
%   {.}% Punteggiatura dopo il titolo dell'enunciato
%   { }% Spazio dopo il titolo dell'enunciato
%   {}% Specifica dell'enunciato

% \theoremstyle{claim}% Imposta lo stile
% \newtheorem{claim}{{\large C}{\footnotesize{LAIM}}}[deff]% Definizione di un nuovo teorema

% \newtheorem{manualtheoreminner}{Theorem}
% \newenvironment{manualtheorem}[1]{%
%   \renewcommand\themanualtheoreminner{#1}%
%   \manualtheoreminner
% }{\endmanualtheoreminner}

% \let\oldrmk=\rmk
% \renewenvironment{rmk}{\begin{oldrmk}}{\hfill$\blacksquare$\end{oldrmk}\\ \par}


% \newenvironment{idea}{\removelastskip\par\medskip   % inizio e fine dimostrazione
% \noindent{\em Idea of the proof} \rm}{\penalty-20\null\hfill$\square$\par\medbreak}

% %%
% %
% %%     SIMBOLI MATEMATICI BLACKBOARD (INSIEMI) R -> \R
% %%
% \newcommand{\N}{\mathbb{N}}
% \newcommand{\Q}{\mathbb{Q}}
% \newcommand{\R}{\mathbb{R}}
% \newcommand{\Z}{\mathbb{Z}}
% %%
% %%

% %%
% %%                          GRECI
% %%
% \newcommand{\aalpha}{{\mbox{\boldmath$\alpha$}}}
% \newcommand{\bbeta}{{\mbox{\boldmath$\beta$}}}
% \newcommand{\ggamma}{{\mbox{\boldmath$\gamma$}}}
% \newcommand{\ddelta}{{\mbox{\boldmath$\delta$}}}
% \newcommand{\eeta}{{\mbox{\boldmath$\eta$}}}
% \newcommand{\llambda}{{\mbox{\boldmath$\lambda$}}}
% \newcommand{\mmu}{{\mbox{\boldmath$\mu$}}}
% \newcommand{\nnu}{{\mbox{\boldmath$\nu$}}}
% \newcommand{\ppi}{{\mbox{\boldmath$\pi$}}}
% \newcommand{\rrho}{{\mbox{\boldmath$\rho$}}}
% \newcommand{\ssigma}{{\mbox{\boldmath$\sigma$}}}
% \newcommand{\ttau}{{\mbox{\boldmath$\tau$}}}
% \newcommand{\pphi}{{\mbox{\boldmath$\phi$}}}
% \newcommand{\ppsi}{{\mbox{\boldmath$\psi$}}}
% \newcommand{\xxi}{{\mbox{\boldmath$ \xi$}}}
% \newcommand{\zzeta}{{\mbox{\boldmath$ \zeta$}}}
% %%
% %%
% \newcommand{\saalpha}{{\mbox{\scriptsize\boldmath$\alpha$}}}
% \newcommand{\sbbeta}{{\mbox{\scriptsize\boldmath$\beta$}}}
% \newcommand{\sggamma}{{\mbox{\scriptsize\boldmath$\gamma$}}}
% \newcommand{\sllambda}{{\mbox{\scriptsize\boldmath$\lambda$}}}
% \newcommand{\smmu}{{\mbox{\scriptsize\boldmath$\mu$}}}
% \newcommand{\snnu}{{\mbox{\scriptsize\boldmath$\nu$}}}
% \newcommand{\sttau}{{\mbox{\scriptsize\boldmath$\tau$}}}
% \newcommand{\seeta}{{\mbox{\scriptsize\boldmath$\eta$}}}
% \newcommand{\sssigma}{{\mbox{\scriptsize\boldmath$\sigma$}}}
% \newcommand{\srrho}{{\mbox{\scriptsize\boldmath$\rho$}}}
% \newcommand{\sppi}{{\mbox{\scriptsize\boldmath$\pi$}}}
% %%
% %% RESTRIZIONE
% %%
% \newcommand{\restr}[1]{\lower3pt\hbox{$|_{#1}$}}
% %%
% %% 
% %% SPAZI MISURE
% %%
% \newcommand{\Mp}{\mathscr M^+}                  % MISURE DI RADON POSITIVE FINITE SUI LIMITATI
% \newcommand{\fm}{{\rm fm}}                              % FINITE MASS
% \newcommand{\pr}{\mathscr P}
% \newcommand{\prd}{\mathscr P_2}
% %%
% %% CURVE
% %%
% \newcommand{\cu}[1]{C([0,1],#1)}
% \newcommand{\geo}{{\rm Geo}}
% \newcommand{\ac}[1]{AC([0,1],#1)}
% \newcommand{\acq}[2]{AC^{#1}([0,1],#2)}
% \newcommand{\keq}[1]{{\sf ke}_{#1}}
% \newcommand{\e}{{\rm e}}
% \newcommand{\et}{{\rm e}_t}
% \newcommand{\ms}{{\sf ms}}
% \newcommand{\Restr}[2]{{\rm Restr}_{#1}^{#2}}


% %%
% %% SPAZI METRICI ECC...
% %%

% \newcommand{\X}{{\rm X}}
% \newcommand{\Y}{{\rm Y}}
% \renewcommand{\Z}{{\rm Z}}


% \newcommand{\XX}{{\sf X}}
% \newcommand{\YY}{{\sf Y}}
% \newcommand{\ZZ}{{\sf Z}}


% \newcommand{\sfd}{{\sf d}}
% \newcommand{\diam}{{\sf diam}}
% \newcommand{\Br}{{\sf Br}}                                                             % Branching geodesics
% %\newcommand{\Cr}{{\sf Cr}}                                                             % Crossing geodesics - 
% \newcommand{\Int}{{\rm Int}}
% \newcommand{\mm}{{\mathfrak m}}
% \newcommand{\mmt}{\tilde{\mathfrak m}}						%m tilde
% \newcommand{\z}{{\sf z}}									%costante rinormalizzazione misure
% \newcommand{\sfC}{{\sf C}}								%costante rinormalizzazione `Gaussiana'
% \newcommand{\zn}{\z_n}									%constante z_n
% \newcommand{\zi}{\z_\infty}								%costante z_\infty
% \newcommand{\gs}{{\sf GeodSel}}							%Geodesic Selection
% \newcommand{\bsr}{{\sf BorSelRep}}							%Borel Selection of Representative (per localizzazione)
% \newcommand{\Par}{{\sf Par}}							%Borel Selection of Representative (per localizzazione)
% \newcommand{\Eu}{{\rm Eu}}								%Euclidean distance (suffisso)




% %%
% %%
% %%   VARIETA'
% %%
% %%

% \newcommand{\ric}{{\rm Ric}}								% Curvatura Ricci
% \newcommand{\riem}{{\rm Riem}}							% Curvatura Riemann
% \newcommand{\vol}{{\rm vol}}								% Misura di volume
% \newcommand{\Tr}{{\rm tr}}								% traccia





% %%
% %% SPAZI FUNZIONALI
% %%
% \renewcommand{\S}{{\rm S}}
% \newcommand{\BV}{{\rm BV}}
% \renewcommand{\L}{{\rm L}} %\renewcommand{\L}{{\sf L}}
% \newcommand{\Lbs}{{\rm Lip}_{\rm bs}}
% \newcommand{\Llo}{{\rm Lip}_{\rm loc}}
% \newcommand{\LIP}{{\rm Lip}}

% %%
% %% CONDIZIONI CURVATURA
% %%
% \newcommand{\CD}{{\sf CD}}
% \newcommand{\CDe}{{\sf CD}^{\rm e}}
% \newcommand{\RCD}{{\sf RCD}}
% \newcommand{\MCP}{{\sf MCP}}
% \newcommand{\snk}{{{\sf{sn}}_k}}
% \newcommand{\sn}[1]{{{\sf{sn}}_{#1}}}
% \newcommand{\sD}{{{\sf{ D}}}}




% %%
% %% FUNZIONALI BASE
% %%
% \newcommand{\ch}{{\sf Ch}}
% \newcommand{\chp}{{\sf Ch}_p}
% \newcommand{\ent}{{\rm Ent}_\mm}
% \newcommand{\entm}[1]{{\rm Ent}_{#1}}
% \newcommand{\U}{{\mathcal U}}               %Funzionale `entropia' generico
% \newcommand{\sfb}{{\sf b}}			%Derivazioni alla Simone
% \newcommand{\apv}{{\rm ApVar}}						% Approximate variation
% \renewcommand{\P}{{\sf P}}							% Perimetro di insiemi di perimetro finito
% \newcommand{\Mink}{{\sf M}}							% Minkowski content (da aggiungere + e - 




% %%
% %% TRASPORTO OTTIMO
% %%
% \newcommand{\opt}{{\sf Opt}}
% \newcommand{\gopt}{{\sf OptGeo}}
% \newcommand{\adm}{{\sf Adm}}
% \newcommand{\W}{{\rm W}}
% \newcommand{\Ib}{{\rm Ib}}   				%INTERPOLATING BOUNDS per densita' geodetiche in CD(K,\infty)
% \newcommand{\nbt}{{\mathcal T}_{\sf nBr}}   				%nonBranching Transport set
% \newcommand{\rel}{{\mathcal Rel}}   						%relazione (indotta da \varphi)


% %%
% %% OPERATORI DIFFERENZIALI
% %%
% \newcommand{\St}{{\rm st}}
% \newcommand{\sta}{{\rm st_a}}
% \newcommand{\Dom}{{\rm D}}
% \renewcommand{\d}{{\rm d}}
% \newcommand{\D}{{\rm D}}		
% \newcommand{\wug}[1]{|{\rm D}_{\rm w}#1|}   				%Weak upper gradient
% \newcommand{\wrs}[1]{|{\rm D}_{\rm r}#1|}				%Weak relaxed slope
% \newcommand{\bvr}[1]{|{\bf D}_{\rm r}#1|}					%minimal relaxed variation
% \newcommand{\bvw}[1]{|{\bf D}_{\rm w}#1|}				%minimal weak variation
% \newcommand{\der}{{\sf Der}}
% \renewcommand{\div}{{\rm div}}
% \newcommand{\lip}{{\rm lip}}
% \newcommand{\Lip}{{\rm Lip}}
% \newcommand{\lipa}{{\rm lip}_a}
% \newcommand{\Hess}{{\rm Hess}}


% %%
% %% LIMITI
% %%

% \newcommand{\lims}{\varlimsup}
% \newcommand{\limi}{\varliminf}

% %%
% %% PEDICI
% %%

% \newcommand{\loc}{{\rm loc}}
% \newcommand{\bs}{{\rm bs}}
% \renewcommand{\b}{{\rm b}}
% \newcommand{\bd}{{\rm bd}}
% \newcommand{\bc}{{\rm bc}}
% \newcommand{\bsbd}{{\rm bsd}}



% %%
% %% VARIE
% %%



% \newcommand{\la}{\langle}
% \newcommand{\ra}{\rangle}
% \renewcommand{\ae}{{\rm a.e.}}
% \newcommand{\weakto}{\rightharpoonup}
% \newcommand{\nchi}{{\raise.3ex\hbox{$\chi$}}}
% \newcommand{\supp}{{\rm supp}}
% \newcommand{\eps}{\varepsilon}
% \newcommand{\Id}{{\rm Id}}
% \newcommand{\fs}{{\sf FinSeq}}				  % Successioni finite (per disintegrazione)
% \newcommand{\B}{\mathcal B}                            % Boreliani
% \renewcommand{\Pr}{{\rm Pr}}				 % Proiezione
% \newcommand{\glimi}{\Gamma-\limi}
% \newcommand{\glims}{\Gamma-\lims}

% \newcommand{\MB}{\it}






% %\newcommand{\st}[1]{\noindent{\bf  #1}}  %per fare step in dimostrazioni

% \newcommand{\Leb}{\mathrm{Leb}}
% \newcommand{\Lu}{\mathcal L_1}  %Lebesgue su [0,1]
% \newcommand{\comp}{{\sf Comp}} %compression constant

% \newcommand{\h}{{\sf h}} % Calore

% \newcommand{\E}{{\sf E}} % Funzionale per gradient flow
% \renewcommand{\sl}[1]{|\partial^-#1|} % Slope del funzionale per gradient flow


% \newcommand{\fr}{\penalty-20\null\hfill$\blacksquare$}         %quadratino nero alla fine del remark

% \newcommand{\tr}[1]{{\text{\rm #1}}}            % per scrivere nelle formule in roman




% \DeclareMathOperator*{\esssup}{\rm ess-sup}
% \DeclareMathOperator*{\essinf}{\rm ess-inf}


% \newcommand\ato[2]{\genfrac{}{}{0pt}{}{#1}{#2}}                %per fare \atop senza incorrere in warning

\newcommand{\bmssd}{\boldsymbol\mssd}

\usepackage{xparse}

\ExplSyntaxOn
%abbreviations
\NewDocumentCommand{\makeabbrev}{mmm}
 {
  \yoruk_makeabbrev:nnn { #1 } { #2 } { #3 }
 }

\cs_new_protected:Npn \yoruk_makeabbrev:nnn #1 #2 #3
 {
  \clist_map_inline:nn { #3 }
   {
    \cs_new_protected:cpn { #2 } { #1 { ##1 } }
   }
 }
 \ExplSyntaxOff
 



 \makeabbrev{\textbf}{tbf#1}{a,b,c,d,e,f,g,h,i,j,k,l,m,n,o,p,q,r,s,t,u,v,w,x,y,z,A,B,C,D,E,F,G,H,I,J,K,L,M,N,O,P,Q,R,S,T,U,V,W,X,Y,Z}

\makeabbrev{\textbf}{bf#1}{a,b,c,d,e,f,g,h,i,j,k,l,m,n,o,p,q,r,s,t,u,v,w,x,y,z,A,B,C,D,E,F,G,H,I,J,K,L,M,N,O,P,Q,R,S,T,U,V,W,X,Y,Z}

\makeabbrev{\textsf}{tsf#1}{a,b,c,d,e,f,g,h,i,j,k,l,m,n,o,p,q,r,s,t,u,v,w,x,y,z,A,B,C,D,E,F,G,H,I,J,K,L,M,N,O,P,Q,R,S,T,U,V,W,X,Y,Z}

\makeabbrev{\mathsf}{mss#1}{a,b,c,d,e,f,g,h,i,j,k,l,m,n,o,p,q,r,s,t,u,v,w,x,y,z,A,B,C,D,E,F,G,H,I,J,K,L,M,N,O,P,Q,R,S,T,U,V,W,X,Y,Z}

\makeabbrev{\mathfrak}{mf#1}{a,b,c,d,e,f,g,h,i,j,k,l,m,n,o,p,q,r,s,t,u,v,w,x,y,z,A,B,C,D,E,F,G,H,I,J,K,L,M,N,O,P,Q,R,S,T,U,V,W,X,Y,Z}

\makeabbrev{\mathrm}{mrm#1}{a,b,c,d,e,f,g,h,i,j,k,l,m,n,o,p,q,r,s,t,u,v,w,x,y,z,A,B,C,D,E,F,G,H,I,J,K,L,M,N,O,P,Q,R,S,T,U,V,W,X,Y,Z}

\makeabbrev{\mathbf}{mbf#1}{a,b,c,d,e,f,g,h,i,j,k,l,m,n,o,p,q,r,s,t,u,v,w,x,y,z,A,B,C,D,E,F,G,H,I,J,K,L,M,N,O,P,Q,R,S,T,U,V,W,X,Y,Z}

\makeabbrev{\mathcal}{mc#1}{A,B,C,D,E,F,G,H,I,J,K,L,M,N,O,P,Q,R,S,T,U,V,W,X,Y,Z}

\makeabbrev{\mathbb}{mbb#1}{A,B,C,D,E,F,G,H,I,J,K,L,M,N,O,P,Q,R,S,T,U,V,W,X,Y,Z}

\makeabbrev{\mathscr}{ms#1}{A,B,C,D,E,F,G,H,I,J,K,L,M,N,O,P,Q,R,S,T,U,V,W,X,Y,Z}

% \makeabbrev{\mathrm}{#1}{
% %Algebraic Ops
% Id,id,ran,rk,diag,stab,ann,conv,pr,ev,tr,End,Hom,sgn,im,op,can,fin,ext,red,tot,
% %
% %Analytic Ops
% rot,usc,lsc,Lip,LocLip,lip,bSymLip,osc,AC,loc,uloc,spec,coz,z,ul,
% %
% %Measure Theory
% supp,Opt,Adm,Cpl,Geo,GeoSel,GeoOpt,GeoAdm,GeoCpl,reg,
% %
% %Topology/Geometry
% bd,co,Ric,Exp,dExp,dist,seg,Seg,cut,fcut,Cut,SDiff,Iso,Isom,diam,cl,Homeo,Diff,Der,vol,dvol,inj,relint, Graph, sub,codim,
% %
% %Probability
% var,law,Poi,Gam,pa,so,iso,fs,inv,pqi,mix,
% %
% TestF,
% %Miscellaneous
% }

% \makeabbrev{\mathsf}{#1}{DP,CD,BE,MCP,Ent,wMTW,MTW,RCD,ncRCD,QCD,EVI,Irr,IH,SC,wFe,VA,UP,Curv,Alex,CAT, Var}


\newcommand{\comma}{\,\,\mathrm{,}\;\,}
\newcommand{\semicolon}{\,\,\mathrm{;}\;\,}
\newcommand{\fstop}{\,\,\mathrm{.}}
\newcommand{\cdc}{\Gamma}   
\newcommand{\Ch}{{\sf Ch}}

\newcommand{\purple}[1]{{\color{purple}#1}}
\newcommand{\blue}[1]{{\color{blue}#1}}
\newcommand{\green}[1]{{\color{OliveGreen}#1}}

\newcommand{\dUpsilon}{{\boldsymbol\Upsilon}}
\newcommand{\U}{\dUpsilon}
\newcommand{\sine}{\mathsf{sine}}
\newcommand{\F}{\mathcal F}
% \newcommand{\p}{\pi}
\newcommand{\CylF}{{\rm Cyl}}
\newcommand{\lab}{\mathfrak l}
\newcommand{\comm}{\,\,\mathrm{,}\;\,}
\newcommand{\cquad}{\comma \quad}
\newcommand{\diff}{\mathrm d}

\newcommand{\e}{\varepsilon}

\newcommand{\defset}[2]{ \left\{ #1 : #2 \right\} }

\newcommand{\mux}{\mfm_{X}}
\newcommand{\muy}{\mfm_{Y}}




\crefname{subsection}{subsection}{subsections}

%%
%% TEOREMI ECC
%%
\numberwithin{equation}{section}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{prop}[theorem]{Proposition}
\AddToHook{env/lemma/begin}{\crefalias{theorem}{lemma}}
\AddToHook{env/proposition/begin}{\crefalias{theorem}{proposition}}
\AddToHook{env/prop/begin}{\crefalias{theorem}{prop}}
\AddToHook{env/corollary/begin}{\crefalias{theorem}{corollary}}



\theoremstyle{definition} \newtheorem{definition}[theorem]{Definition}

\theoremstyle{definition}  \newtheorem{setting}[theorem]{Setting}
\theoremstyle{definition}  \newtheorem{example}[theorem]{Example}
\theoremstyle{definition}  \newtheorem{remark}[theorem]{Remark}
\newtheorem{exercise}[theorem]{Exercise}
\theoremstyle{definition}  \newtheorem{open}[theorem]{Open problem}
\newtheorem{thmdef}[theorem]{Theorem/Definition}
\theoremstyle{definition}  \newtheorem{ass} [theorem]{Assumption}

\AddToHook{env/definition/begin}{\crefalias{theorem}{definition}}
\AddToHook{env/setting/begin}{\crefalias{theorem}{setting}}
\AddToHook{env/example/begin}{\crefalias{theorem}{example}}
\AddToHook{env/remark/begin}{\crefalias{theorem}{remark}}
\AddToHook{env/ass/begin}{\crefalias{theorem}{ass}}
\AddToHook{env/exercise/begin}{\crefalias{theorem}{exercise}}
\AddToHook{env/thmdef/begin}{\crefalias{theorem}{thmdef}}

\newenvironment{idea}{\removelastskip\par\medskip   % inizio e fine dimostrazione
\noindent{\em Idea of the proof} \rm}{\penalty-20\null\hfill$\square$\par\medbreak}


%%
%
%%     SIMBOLI MATEMATICI BLACKBOARD (INSIEMI) R -> \R
%%
\newcommand{\N}{\mathbb{N}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\Mn}{\mathbb R^{1,n}}
%%
%%

%%
%%                          GRECI
%%
\newcommand{\aalpha}{{\mbox{\boldmath$\alpha$}}}
\newcommand{\bbeta}{{\mbox{\boldmath$\beta$}}}
\newcommand{\ggamma}{{\mbox{\boldmath$\gamma$}}}
\newcommand{\ddelta}{{\mbox{\boldmath$\delta$}}}
\newcommand{\eeta}{{\mbox{\boldmath$\eta$}}}
\newcommand{\llambda}{{\mbox{\boldmath$\lambda$}}}
\newcommand{\mmu}{{\mbox{\boldmath$\mu$}}}
\newcommand{\nnu}{{\mbox{\boldmath$\nu$}}}
\newcommand{\ppi}{{\mbox{\boldmath$\pi$}}}
\newcommand{\rrho}{{\mbox{\boldmath$\rho$}}}
\newcommand{\ssigma}{{\mbox{\boldmath$\sigma$}}}
\newcommand{\ttau}{{\mbox{\boldmath$\tau$}}}
\newcommand{\pphi}{{\mbox{\boldmath$\phi$}}}
\newcommand{\ppsi}{{\mbox{\boldmath$\psi$}}}
\newcommand{\xxi}{{\mbox{\boldmath$ \xi$}}}
\newcommand{\zzeta}{{\mbox{\boldmath$ \zeta$}}}
%%
%%
\newcommand{\saalpha}{{\mbox{\scriptsize\boldmath$\alpha$}}}
\newcommand{\sbbeta}{{\mbox{\scriptsize\boldmath$\beta$}}}
\newcommand{\sggamma}{{\mbox{\scriptsize\boldmath$\gamma$}}}
\newcommand{\sllambda}{{\mbox{\scriptsize\boldmath$\lambda$}}}
\newcommand{\smmu}{{\mbox{\scriptsize\boldmath$\mu$}}}
\newcommand{\snnu}{{\mbox{\scriptsize\boldmath$\nu$}}}
\newcommand{\sttau}{{\mbox{\scriptsize\boldmath$\tau$}}}
\newcommand{\seeta}{{\mbox{\scriptsize\boldmath$\eta$}}}
\newcommand{\sssigma}{{\mbox{\scriptsize\boldmath$\sigma$}}}
\newcommand{\srrho}{{\mbox{\scriptsize\boldmath$\rho$}}}
\newcommand{\sppi}{{\mbox{\scriptsize\boldmath$\pi$}}}
%%
%% RESTRIZIONE
%%
\newcommand{\restr}[1]{\lower3pt\hbox{$|_{#1}$}}
%%
%% 
%% SPAZI MISURE
%%
\newcommand{\Mp}{\mathscr M^+}                  % MISURE DI RADON POSITIVE FINITE SUI LIMITATI
\newcommand{\M}{\mathscr M}    
\newcommand{\fm}{{\rm fm}}                              % FINITE MASS
\newcommand{\pr}{\mathscr P}
\newcommand{\prd}{\mathscr P_2}
%%
%% CURVE
%%
\newcommand{\cu}[1]{C([0,1],#1)}
\newcommand{\geo}{{\rm Geo}}
\newcommand{\ac}[1]{AC([0,1],#1)}
\newcommand{\acq}[2]{AC^{#1}([0,1],#2)}
\newcommand{\keq}[1]{{\sf ke}_{#1}}
% \newcommand{\e}{{\rm e}}
\newcommand{\et}{{\rm e}_t}
\newcommand{\ms}{{\sf ms}}
% \newcommand{\Restr}[2]{{\rm Restr}_{#1}^{#2}}
\newcommand{\Restr}{{\mathrm{restr}}}


%%
%% SPAZI METRICI ECC...
%%

\newcommand{\X}{{\rm X}}
\newcommand{\Y}{{\rm Y}}
\renewcommand{\Z}{{\rm Z}}
\newcommand{\p}{{\sf p}}


\newcommand{\XX}{{\sf X}}
\newcommand{\YY}{{\sf Y}}
\newcommand{\ZZ}{{\sf Z}}


\newcommand{\sfd}{{\sf d}}
\newcommand{\diam}{{\sf diam}}
\newcommand{\Br}{{\sf Br}}                                                             % Branching geodesics
%\newcommand{\Cr}{{\sf Cr}}                                                             % Crossing geodesics - 
\newcommand{\Int}{{\rm Int}}
\newcommand{\mm}{{\mathfrak m}}
\newcommand{\mmt}{\tilde{\mathfrak m}}						%m tilde
\newcommand{\z}{{\sf z}}									%costante rinormalizzazione misure
\newcommand{\sfC}{{\sf C}}								%costante rinormalizzazione `Gaussiana'
\newcommand{\zn}{\z_n}									%constante z_n
\newcommand{\zi}{\z_\infty}								%costante z_\infty
\newcommand{\gs}{{\sf GeodSel}}							%Geodesic Selection
\newcommand{\bsr}{{\sf BorSelRep}}							%Borel Selection of Representative (per localizzazione)
\newcommand{\Par}{{\sf Par}}							%Borel Selection of Representative (per localizzazione)
\newcommand{\Eu}{{\rm Eu}}								%Euclidean distance (suffisso)

\newcommand{\LCC}{\mathrm{LCC}}

\newcommand{\eval}{\mathsf{e}}




%%
%%
%%   VARIETA'
%%
%%

\newcommand{\ric}{{\rm Ric}}								% Curvatura Ricci
\newcommand{\riem}{{\rm Riem}}							% Curvatura Riemann
\newcommand{\vol}{{\rm vol}}								% Misura di volume
\newcommand{\Tr}{{\rm tr}}								% traccia





%%
%% SPAZI FUNZIONALI
%%
\renewcommand{\S}{{\rm S}}
\newcommand{\BV}{{\rm BV}}
\renewcommand{\L}{{\rm L}} %\renewcommand{\L}{{\sf L}}
\newcommand{\Lbs}{{\rm Lip}_{\rm bs}}
\newcommand{\Llo}{{\rm Lip}_{\rm loc}}
\newcommand{\LIP}{{\rm Lip}}
\newcommand{\scrC}{\mathscr{C}}

%%
%% CONDIZIONI CURVATURA
%%
\newcommand{\CD}{{\sf CD}}
\newcommand{\CDe}{{\sf CD}^{\rm e}}
\newcommand{\RCD}{{\sf RCD}}
\newcommand{\MCP}{{\sf MCP}}
\newcommand{\snk}{{{\sf{sn}}_k}}
\newcommand{\sn}[1]{{{\sf{sn}}_{#1}}}
\newcommand{\sD}{{{\sf{ D}}}}




%%
%% FUNZIONALI BASE
%%
\newcommand{\ch}{{\sf Ch}}
\newcommand{\chp}{{\sf Ch}_p}
\newcommand{\ent}{{\rm Ent}_\mm}
\newcommand{\entm}[1]{{\rm Ent}_{#1}}
% \newcommand{\U}{{\mathcal U}}               %Funzionale `entropia' generico
\newcommand{\sfb}{{\sf b}}			%Derivazioni alla Simone
\newcommand{\apv}{{\rm ApVar}}						% Approximate variation
\renewcommand{\P}{{\sf P}}							% Perimetro di insiemi di perimetro finito
\newcommand{\Mink}{{\sf M}}							% Minkowski content (da aggiungere + e - 




%%
%% TRASPORTO OTTIMO
%%
\newcommand{\opt}{{\sf Opt}}
\newcommand{\gopt}{{\sf OptGeo}}
\newcommand{\adm}{{\sf Adm}}
\newcommand{\W}{{\rm W}}
\newcommand{\Ib}{{\rm Ib}}   				%INTERPOLATING BOUNDS per densita' geodetiche in CD(K,\infty)
\newcommand{\nbt}{{\mathcal T}_{\sf nBr}}   				%nonBranching Transport set
\newcommand{\rel}{{\mathcal Rel}}   						%relazione (indotta da \varphi)


%%
%% OPERATORI DIFFERENZIALI
%%
\newcommand{\bs}{\partial^{\sf b}}
\newcommand{\fs}{\partial^{\sf f}}
\DeclareMathOperator{\St}{St}
\DeclareMathOperator{\stp}{st}
\newcommand{\sta}{{\rm st_a}}
\newcommand{\Dom}{{\mathscr{D}}}
\renewcommand{\d}{{\rm d}}
\newcommand{\D}{{\rm D}}		
\newcommand{\wug}[1]{|{\rm D}_{\rm w}#1|}   				%Weak upper gradient
\newcommand{\wrs}[1]{|{\rm D}_{\rm r}#1|}				%Weak relaxed slope
\newcommand{\bvr}[1]{|{\bf D}_{\rm r}#1|}					%minimal relaxed variation
\newcommand{\bvw}[1]{|{\bf D}_{\rm w}#1|}				%minimal weak variation
\newcommand{\der}{{\sf Der}}
\renewcommand{\div}{{\rm div}}
\newcommand{\lip}{{\rm lip}}
\newcommand{\Lip}{{\rm Lip}}
\newcommand{\lipa}{{\rm lip}_a}
\newcommand{\Hess}{{\rm Hess}}


%%
%% LIMITI
%%

\newcommand{\lims}{\varlimsup}
\newcommand{\limi}{\varliminf}
\newcommand{\concto}{\xrightarrow{{\sf conc}}}

%%
%% PEDICI
%%

\newcommand{\loc}{{\rm loc}}
% \newcommand{\bs}{{\rm bs}}
\renewcommand{\b}{{\rm b}}
\newcommand{\bd}{{\rm bd}}
\newcommand{\bc}{{\rm bc}}
\newcommand{\bsbd}{{\rm bsd}}



%%
%% VARIE
%%


\newcommand{\Leb}{\mathscr{L}}
\renewcommand{\ae}{{\rm a.e.}}
\newcommand{\weakto}{\rightharpoonup}
\newcommand{\nchi}{{\raise.3ex\hbox{$\chi$}}}
\newcommand{\supp}{{\rm supp}}
\newcommand{\eps}{\varepsilon}
\newcommand{\Id}{{\rm Id}}
% \newcommand{\fs}{{\sf FinSeq}}				  % Successioni finite (per disintegrazione)
\newcommand{\B}{\mathcal B}                            % Boreliani
\renewcommand{\Pr}{{\rm Pr}}				 % Proiezione
\newcommand{\proj}{{\rm proj}}				 % Proiezione
\newcommand{\sfQ}{\mathsf{Q}}
\newcommand{\rmD}{\mathrm{D}}
\newcommand{\RSS}{{\sf RSS}}
\newcommand{\One}{\mathbbm{1}}
\newcommand{\mres}{\mathbin{\vrule height 1.6ex depth 0pt width 0.13ex\vrule height 0.13ex depth 0pt width 1.3ex}}

\newcommand{\HH}{\mathsf{h}}






%\newcommand{\st}[1]{\noindent{\bf  #1}}  %per fare step in dimostrazioni


\newcommand{\Lu}{\mathcal L_1}  %Lebesgue su [0,1]
\newcommand{\comp}{{\sf Comp}} %compression constant

\newcommand{\h}{{\sf h}} % Calore

\newcommand{\E}{{\sf E}} % Funzionale per gradient flow
% \newcommand{\F}{{\mathcal F}} % Funzionale F
\renewcommand{\sl}[1]{|\partial^-#1|} % Slope del funzionale per gradient flow


\newcommand{\fr}{\penalty-20\null\hfill$\blacksquare$}         %quadratino nero alla fine del remark

\newcommand{\tr}[1]{{\text{\rm #1}}}            % per scrivere nelle formule in roman




\DeclareMathOperator*{\esssup}{\rm ess-sup}
\DeclareMathOperator*{\essinf}{\rm ess-inf}


\newcommand\ato[2]{\genfrac{}{}{0pt}{}{#1}{#2}}                %per fare \atop senza incorrere in warning

\newcommand{\TBD}[1]{\textcolor{red}{#1}} %to be done
\newcommand{\bookmark}{\par\noindent\rule{\linewidth}{0.4pt}\par}

\newcommand{\cyan}{\textcolor{cyan}}
\newcommand{\essup}{\mathrm{ess\text{-}sup}}
\newcommand{\med}{\mathsf{med}}
% \mathtoolsset{
% 	showonlyrefs
% }
\usepackage{pdflscape}
\usepackage{booktabs}
\usepackage{array}
\usepackage{adjustbox}
%\newcommand{\blue}{\textcolor{blue}}
\usepackage{pdflscape,booktabs,tabularx,array}
%\newcommand{\purple}{\textcolor{purple}}

\newcommand{\ppr}{{\rm pr}}

\newcommand{\sfp}{\mathsf p}


